A Survey for H$_2$O Megamasers in Active Galactic Nuclei -- II. A Comparison of Detected and Undetected Galaxies

A survey for H2O megamaser emission from 354 active galaxies has resulted in the detection of 10 new sources, making 16 known altogether. The galaxies surveyed include a distance-limited sample (covering Seyferts and LINERs with recession velocities < 7000 km s^{-1}) and a magnitude-limited sample (covering Seyferts and LINERs with m(B) <= 14.5). In order to determine whether the H2O-detected galaxies are "typical" AGN or have special properties which facilitate the production of powerful masers, we have accumulated a database of physical, morphological, and spectroscopic properties of the observed galaxies. The most significant finding is that H2O megamasers are detected only in Seyfert 2 and LINER galaxies, not Seyfert 1s. Implications for this finding are discussed. LINERs are detected at a similar rate to Seyfert 2s, constituting a strong argument that at least some nuclear LINERs are AGN rather than starbursts, since starbursts have not been detected as H2O megamasers. We preferentially detect H2O emission from the nearer galaxies and from those which are apparently brighter at mid- and far-infrared and centimeter radio wavelengths. There is also a possible trend for the H2O-detected galaxies to be more intrinsically luminous in nuclear 6 cm radio emission than the undetected ones, though these data are incomplete. We find evidence that Seyfert 2s with very high (N(H) > 10^{24} cm^{-2}) X-ray absorbing columns of gas are more often detected as H2O maser emitters than Seyfert 2s with lower columns. It may be that the probability of detecting H2O maser emission in Seyfert galaxies increases with increasing column of cool gas to the nucleus, from Seyfert 1s through NLXGs to Seyfert 2s.

==> braatz-figcap.tex <==
\def\sollum {\hbox{$L_{\odot}$}}
\def\lesssim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$<$}}}}
\def\gtrsim{\mathrel{\hbox{\rlap{\hbox{\lower4pt\hbox{$\sim$}}}\hbox{$>$}}}}
\def\arcsec {\hbox{$^{\prime\prime}$}}
\def\deg{\ifmmode^\circ\else$^\circ$\fi}
\magnification =\magstep1
\nopagenumbers

\bigskip
\noindent
Figure 1.  The positions of all observed galaxies are plotted
in Galactic coordinates using the Aitoff projection.  Equal areas on this plot
correspond to equal areas on the sky.  Galaxies detected in H$_2$O are
shown as filled circles, undetected galaxies which are a member of
either the distance- or magnitude-limited sample are represented by
diamonds, and other undetected galaxies are shown as squares.  The Galactic 
center is at the origin in the middle of the plot.

\bigskip
\noindent
Figure 2.  The distribution of recession velocity for the detected and
undetected galaxies are compared.  The undetected galaxies in the
sensitivity-limited sample are represented by the dark shaded region.  They
make up a subset of the undetected galaxies in the distance-limited
sample, which are represented by the lighter shaded region.  The
undetected galaxies in the magnitude-limited
sample are plotted as filled triangles.  These data are scaled
according to the left axis.  The detected galaxies are represented by vertical
bars, and they are plotted using the magnified scale shown on the right axis.
The entire set of observed
galaxies (detected and undetected) is represented by the open squares, and are
plotted according to the scale on the left axis.
All histograms in this chapter follow a scheme similar to this one.

\bigskip
\noindent
Figure 3.  The values of $<V/V_{max}>$ are plotted as a function of
recession velocity for galaxies in the distance-limited sample.
The open markers show $<V/V_{max}>$ for the individual AGN classes, according
to the legend, and the filled squares show the complete distance-limited sample.  

\bigskip
\noindent
Figure 4.  The values of $<V/V_{max}>$ are plotted as a function of B
magnitude for galaxies in the magnitude-limited sample.
The open markers show $<V/V_{max}>$ for the individual AGN classes, according
to the legend, and the filled squares show the complete magnitude-limited
sample.  

\bigskip
\noindent
Figure 5.  The distribution of galactic inclinations for the
distance-limited sample is compared to the inclinations of randomly
oriented thin disks. 

\bigskip
\noindent
Figure 6.  The distributions of the integrated apparent magnitude, m$_B$,
of the detected and undetected galaxies are compared.
Magnitudes are not corrected for Galactic or internal extinction.

\bigskip
\noindent
Figure 7.  The distributions of the integrated absolute magnitude, M$_B$,
of the detected and undetected galaxies are compared.
Magnitudes are calculated from the apparent
face-on magnitude, corrected for Galactic and internal extinction.

\bigskip
\noindent
Figure 8.  The distributions of Hubble stage index for the detected and
undetected galaxies are compared.  The definition and values of $T$
are taken from RC3.

\bigskip
\noindent
Figure 9.  The distributions of inclination (in degrees) of the
detected and undetected galaxies are compared.
Elliptical galaxies ($T$ $\le$ --3) are omitted from this histogram.

\bigskip
\noindent
Figure 10.  The distribution of inclination (in degrees) is shown
for the three AGN classes individually.  The vertical bars represent the 
detected
galaxies and the lines show the distributions for undetected galaxies in the 
distance-limited sample.  Elliptical galaxies
($T$ $\le$ --3) are omitted from this histogram.

\bigskip
\noindent
Figure 11.  Isotropic maser luminosity (in $\sollum$)
is plotted against galactic inclination (in degrees).
The luminosities plotted here are representative values taken from Table 2
of Paper I and are assigned a nominal uncertainty of 25\%. 
The elliptical galaxy NGC 1052 is not included in this figure.

\bigskip
\noindent
Figure 12.  A representative peak maser luminosity
(in $\sollum (km s^{-1})^{-1}$) is plotted against
inclination (in degrees) for each of the detected galaxies.  The
luminosities are calculated from the peak maser fluxes listed in Table 2
of Paper I.
Peak maser luminosities, being extremely variable, are plotted with arbitrary
50\% error bars.  The elliptical galaxy NGC 1052 is not included in this figure.

\bigskip
\noindent
Figure 13.  The distributions of the 12 $\mu m$ flux, S(12) (in Jy), from
IRAS for the detected and undetected galaxies are compared.

\bigskip
\noindent
Figure 14.  The distributions of the 12 $\mu m$ power, P(12) (in 
W Hz$^{-1}$), from IRAS for the detected and undetected galaxies are compared.

\bigskip
\noindent
Figure 15.  The distributions of the 25 $\mu m$ flux, S(25) (in Jy), from
IRAS for the detected and undetected galaxies are compared.

\bigskip
\noindent
Figure 16.  The distributions of the 25 $\mu m$ power, P(25) (in 
W Hz$^{-1}$), from IRAS for the detected and undetected galaxies are compared.

\bigskip
\noindent
Figure 17.  The distributions of the 60 $\mu m$ flux, S(60) (in Jy), from
IRAS for the detected and undetected galaxies are compared.

\bigskip
\noindent
Figure 18.  The distributions of the 60 $\mu m$ power, P(60) (in 
W Hz$^{-1}$), from IRAS for the detected and undetected galaxies are compared.

\bigskip
\noindent
Figure 19.  The distributions of the 100 $\mu m$ flux, S(100) (in Jy), from
IRAS for the detected and undetected galaxies are compared.

\bigskip
\noindent
Figure 20.  The distributions of the 100 $\mu m$ power, P(100) (in 
W Hz$^{-1}$), from IRAS for the detected and undetected galaxies are compared.

\bigskip
\noindent
Figure 21.  The log of the 60 $\mu m$ flux is plotted against the log
of the 25 $\mu m$ flux for all galaxies detected at both 25 and 60 $\mu m$
in the distance-limited and H$_2$O maser detected samples.
AGN classes are differentiated according to the symbols defined in the legend.

\bigskip
\noindent
Figure 22.  The far-IR color S(60 $\mu m$)/S(100 $\mu m$) is plotted against
the mid-IR color S(12 $\mu m$)/S(25 $\mu m$) for each
galaxy in the distance-limited sample and for each galaxy with detected H$_2$O 
megamaser emission.

\bigskip
\noindent
Figure 23.  The distributions of the S(60 $\mu m$)/S(100 $\mu m$) IRAS
flux ratio for the detected and undetected galaxies are compared.

\bigskip
\noindent
Figure 24.  The IR color S(25 $\mu m$)/S(60 $\mu m$) is plotted against
the power in the 25 $\mu m$ IRAS band (in W Hz$^{-1}$) for each galaxy in the
distance-limited sample and for the H$_2$O detected galaxies.  

\bigskip
\noindent
Figure 25.  The distributions of the S(25 $\mu m$)/S(60 $\mu m$) IRAS
flux ratio for the detected and undetected galaxies are compared.

\bigskip
\noindent
Figure 26.  The distributions of small aperture ($\lesssim$ 15\arcsec)
measurements of apparent V magnitude for the detected and undetected
galaxies are compared.

\bigskip
\noindent
Figure 27.  The distributions of absolute nuclear V magnitude for the
detected and undetected galaxies are compared.  The magnitudes
have been calculated from small aperture ($\lesssim$ 15\arcsec) measurements.

\bigskip
\noindent
Figure 28.  The distributions of the log of the nuclear 6 cm radio flux (in mJy)
for the detected and undetected galaxies are compared.

\bigskip
\noindent
Figure 29.  The distributions of the log of the nuclear 6 cm radio power
(in W Hz$^{-1}$) for the detected and undetected galaxies are compared.

\bigskip
\noindent
Figure 30.  The distributions of the log of the [OIII] $\lambda$5007 flux
(in erg cm$^{-2}$ s$^{-1}$) for the detected and undetected galaxies
are compared.

\bigskip
\noindent
Figure 31.  The distributions of the log of the [OIII] $\lambda$5007
luminosity (in erg s$^{-1}$) for the detected and undetected galaxies 
are compared.

\bigskip
\noindent
Figure 32.  The ratio [OIII] $\lambda$5007/H$\beta$ is plotted against
the [OIII] $\lambda$5007 luminosity (in erg s$^{-1}$)
for the maser-detected galaxies and galaxies in the distance-limited sample.

\bigskip
\noindent
Figure 33.  The X-ray luminosity in the 2 -- 10 keV band (in erg s$^{-1}$)
is plotted against the isotropic maser luminosity (in $\sollum$)
for the six maser-detected galaxies with available hard X-ray luminosities.

\bigskip
\noindent
Figure 34.  The equivalent hydrogen column density N$_H$ (in cm$^{-2}$), 
determined by model
fits to the X-ray spectrum, is plotted against the isotropic maser luminosity
(in $\sollum$) for the nine maser-detected galaxies with available column
densities.

\bigskip
\noindent
Figure 35.  The data for this histogram of column densities N$_H$ (in cm$^{-2}$)
of ASCA-observed Seyfert 2 galaxies is taken from Awaki (1996).  We
have shaded the H$_2$O maser-detected sources.  The arrow (and bin separation
at log N$_H$ = 24)
indicates that all sources with N$_H$ $>$ 10$^{24}$ cm$^{-2}$ are plotted
in the rightmost bin.
\end

